Evaluating the Impact of Flaky Simulators on Testing Autonomous Driving Systems

Simulators are widely used to test Autonomous Driving Systems (ADS), but their potential flakiness can lead to inconsistent test results. We investigate test flakiness in simulation-based testing of ADS by addressing two key questions: (1) How do flaky ADS simulations impact automated testing that relies on randomized algorithms? and (2) Can machine learning (ML) effectively identify flaky ADS tests while decreasing the required number of test reruns? Our empirical results, obtained from two widely-used open-source ADS simulators and five diverse ADS test setups, show that test flakiness in ADS is a common occurrence and can significantly impact the test results obtained by randomized algorithms. Further, our ML classifiers effectively identify flaky ADS tests using only a single test run, achieving F1-scores of $85$%, $82$% and $96$% for three different ADS test setups. Our classifiers significantly outperform our non-ML baseline, which requires executing tests at least twice, by $31$%, $21$%, and $13$% in F1-score performance, respectively. We conclude with a discussion on the scope, implications and limitations of our study. We provide our complete replication package in a Github repository.

==> answerMajorReview.tex <==
%%%%
%%% COMMAND USAGE:
%%% REPORTING THE COMMENT
%%% \rwcomment{commentid}{comment textual description}
%%% commentid -> an id of your choice associated with the comment
%%% comment textual descriptionn -> the original comment of the reviewer

%%% ANSWERING A COMMENT
%%% \response{The response for the question. If you want to reference some text use \referenceaddressed{idAssociated with the answer in the text of the paper}}

%%% CHANGING THE PAPER CONTENT
%% \change{new text that will be added}{identifier of the answer choosen by you to be used within the response command in the referenceaddress macro}{identifier of the reviewer comment}
%% \delete{text to be deleted}}{identifier of the answer choosen by you to be used within the response command in the referenceaddress macro}{identifier of the reviewer comment}
%% \rep{new text}{old text}{identifier of the answer choosen by you to be used within the response command in the referenceaddress macro}{identifier of the reviewer comment}

\noindent\textbf{Associate Editor}
\vspace*{.5cm}
\rwcomment{ARC1}{Strengthen the focus on “flakiness” (R1, R2). In particular, address the concern of R1 expressed in relation to RQ1-2}
\response{We have now significantly extended, improved and restructured the discussion section (Section~\ref{sec:conclusion}). Our revision aims to (1) provide a more detailed insight into the potential causes of flakiness and its associated impacts, and (2) present three lessons derived directly from our experimental results, highlighting the characteristics of test inputs, ADS controllers and simulators that contribute to flakiness. Further, as requested by a comment on RQ1-2 from  Reviewer~\#1, we have now updated Table~\ref{tab:variations-carla} to include the frequency of the observed inconsistencies across flaky simulations.}


\rwcomment{ARC2}{Improve the presentation (R1, R2, R3). This could be done, for example, by simple visual enhancements (see R2) or by restructuring the text that presents results (see R1).}
\response{We have substantially improved the presentation of our paper. The specific improvements are as follows:  (1)~We revised and ensured the readability of all figures, tables, and algorithms. (2) We divided Section~\ref{sec:eval} into multiple subsections and used lists with proper indentation to present items. (3) We have improved and restructured the motivation for RQ1-1 to RQ1-3 to better clarify the purpose of each research question.  (4) We added Table~\ref{tab:expinfo} to clearly describe the characteristics of the ADS test setups used in our experiments. (5) We included summary sentences in the evaluation section to enhance readability.  (6) We have added Table~\ref{tab:finalres} to our discussion (Section~\ref{sec:conclusion}) to summarize the results that are used as a basis to derive the lessons learned. (7) We addressed all specific presentation issues raised by the three reviewers.}

\rwcomment{ARC3}{Reviewer R3 raises an interesting concern regarding the relevance of the chosen simulator. While CARLA seems to be widely used in academia, it might not be relevant to the automotive industry where typically proprietary simulators are used. Thus, the relevance of your results to industry needs some additional explanation.}
\response{Thank you for the comment. The  CARLA simulator, in addition to be widely-used in academia, has received endorsements from large companies such as Benz, Huawei, and Samsung~\cite{carlawebsite}, and is sponsored by Intel, NVIDIA, and Toyota~\cite{carlaservices}. 
In addition, we note that potential flakiness of simulators for robotics and cyber-physical systems is a known problem. A recent industry survey lists simulation flakiness as a major challenge for robotic simulators~\cite{afsoon-robotics}. \\
%Considering the extensive use of CARLA and BeamNG in current research, dismissing our work for using these two simulators would suggest that a vast body of existing research is also irrelevant.\\
That being said, we would like to emphasize that our study's findings are not meant to criticize BeamNG and CARLA. As we discuss in Section~\ref{sec:conclusion} under the \emph{Clarification of the Scope} item, many factors may contribute to the flakiness of simulators. Some of these factors, such as uncertainties in the physical models of simulators, are inherent to the physics-based design of both commercial and open-source simulators, and hence may be inevitable.\\
Finally, the main conclusion of our work is that the methods employed in the software engineering literature for assessing simulation-based ADS testing approaches may  lack robustness and may be unreliable  due to the flakiness of ADS simulators. As we discuss in Section~\ref{sec:conclusion} under the \emph{Implications of Our Results} item, we either need to consider restricted ADS test setups where the flakiness is negligible, or we need to develop an evaluation  method that is not sensitive to flakiness. We have updated our paper with this discussion on~\referenceaddressed{R3C1-intro}. }



\newpage

\noindent\textbf{Reviewer \#1} 

\rwcomment{R1C1}{The paper admits that the ADS itself can rely on machine
learning and deep neural networks, which would make these systems naturally
stochastic and nondeterministic in nature. How do we know whether the flakiness
comes from the ADS itself or the simulator being used to test the ADS? Knowing
the source of flakiness at this level can help us better understand what to
focus on when trying to mitigate flakiness, whether it is something to watch
out from in the ADS (which may indicate some true nondeterministic bugs that
should be addressed) or from the simulator having nondeterministic executions.
}
\response{Thank you for the comment. We would like to clarify that, in the case of our deep learning-based ADS models, i.e., Pylot and Transfuser, we have not detected any non-determinism during the inference phase. Hence, we believe that, in our experiments, the ADS itself is not a contributor to the observed flakiness. \\
We identify two main sources of flakiness in our study: The simulator's behaviour, e.g., uncertainties in simulator physical models, and the randomness in the interactions between the simulator and the ADS. The latter is often due to inconsistent timing and synchronization between the ADS and the simulator or due to the white noise added by the simulator to images,  leading the simulator to relay slightly different images to the ADS over different executions. We have addressed and clarified that the ADS itself is not a source of flakiness in our experiments  on \referenceaddressed{R1C1l2} and \referenceaddressed{R1C1L1}. }

\rwcomment{R1C2}{I feel like RQ1-2 is trying to go into this aspect, and I appreciate the manual
inspection gone into why there are flaky failures, but I feel this section can
be expanded much more. Also, concerning RQ1-2, it seems the evaluation was done via
manual inspection of 40 tests, but Table 3 only describes 12 inconsistencies. I
assume multiple tests fall under the same inconsistency, but the table does not
give a sense of how many under each one I feel like inconsistencies of Type I
and II are more due to simulator flakiness while Type III are more due to ADS
nondeterminism, so knowing just how many tests fall under each type would give
a better sense of the prevalence of flakiness in simulators.}
\response{Thank you for the comment. We have now updated Table~\ref{tab:variations-carla} by adding a column to indicate the number of occurrences of each inconsistency. We agree with your observation that the type I and II variations are likely related to the simulator, while type III variations are likely a result of synchronization timing inconsistencies between the simulator and the ADS or are due to the white noise addition. This observation is indeed consistent with the results shown in Table~\ref{tab:variations-carla}. Specifically, Table~\ref{tab:variations-carla} shows that the \textsc{PID} setup, which uses the simulator's PID controller as ADS, exhibits the observed type I and II variations. This supports our hypothesis that the simulator’s autopilot, specifically Carla PID, is the source of these inconsistencies.   In contrast,  most type III inconsistencies are related to the \textsc{Pylot} setup, which uses an external DNN-enabled ADS, and is prone to issues caused by the timing inconsistencies between the ADS and the simulator and the white noise addition.  We have now updated our paper with this discussion on~\referenceaddressed{R1C2ll}
}


%We clarify that the main purpose of RQ1-2 is to  determine whether the re-executions of flaky tests represent fundamentally flawed scenarios, or whether, despite generating different fitness values, these re-executions still represent valid  driving scenarios. The conclusion is that among the 40 randomly selected flaky test samples, only one sample exhibits totally infeasible and flawed  reruns, and the reruns of the remaining  samples are reasonable and, independently, realistic. While RQ1-2 offers insights into the variations caused by the flakiness of simulator-based testing of ADS, we believe that it is not sufficient to draw conclusions on the root causes of flakiness solely based on the results presented in Table~\ref{tab:variations-carla}.

\rwcomment{R1C3}{There are many details in the discussion section that
goes into various reasons for flakiness, but they seem rather high-level and
hypothetical. I would appreciate if such discussion can also be connected more
with the results found in the study as to have greater evidence for these
observations.}
\response{We have now extended, improved and restructured the discussion section (Section~\ref{sec:conclusion}). Specifically, that section provides three lessons, two of which are new in this revision. As we now clarify,  these three lessons are not hypothetical and explicitly build on the results of our experiments. The lessons are as follows: (1)~The lane-keeping test setup shows the lowest rate of flaky tests, (2)~Modular DNN-enabled ADS reduces flaky tests compared to end-to-end DNN-enabled ADS, and (3)~The Carla simulator yields a lower flaky test  rate compared to the BeamNG simulator.  In addition, Section~\ref{sec:conclusion} includes two clarifications related to the scope and the implications of our work, and our observations as to how our experiments may influence the research on ADS testing.  
Please see the updates related to this comment on~\referenceaddressed{R1C7L1}}

\rwcomment{R1C4}{The current way used to evaluate the ML approach seems to follow standard
practice of breaking apart the data into training and evaluation sets in a
cross-fold evaluation. However, this evaluation methodology does not reflect
how one would use the ML approach in practice. I imagine that the main use
scenario is to train a model on many examples across different ADSs, and this
model should be general enough to be used for speeding up flaky-test prediction
for tests of a different ADS, i.e., training a model that can be reused by
other developers for their own projects. In the current setup, the model is
trained using tests from an ADS that is also used for the evaluation, which
does not match this use scenario of a developer reusing a trained model for
their own system. Another way of doing the training and evaluation is to break
apart the data based on the ADS each data point comes from, to train on data
from all ADSs but one and then evaluate on all the data from that remaining ADS
that was not used during training. This is a sort of per-project evaluation
that has been used in other work in flaky-test prediction techniques (see
reference below). Alternatively, another reasonable use scenario is to train on
all data from a single ADS with the intent to reuse that model on future tests
for the same ADS (so the goal is not to create a general model that works for
any system but one dedicated for a specific system). If so, such an evaluation
should train and evaluate on data from a single ADS. I would like to see
whether the machine learning approach can be shown similarly as effective in
these methodologies that better match the intended use scenario.}
\response{Thank you for the comment. We note that as discussed in \referenceaddressed{R1C1l2}, based on our observations, the root-causes of flakiness are related to the simulator or to the interactions between the ADS and the simulator. Hence, flakiness predictors may not generalize beyond a simulator or even a pair of simulator and ADS. Therefore,  in this domain, it seems more reasonable to train a predictor for each pair of simulator and ADS. This is the approach taken in our experiments in training ML models. This allows the developers that use the same simulator and ADS, e.g. CARLA with Pylot, use our pre-trained flakiness predictors in order to optimize the number of reruns for each scenario. We have now added this discussion on~\referenceaddressed{R1C8L1}} 
%Another possibility is to train a flakiness predictor for each Simulator-ADS pair with our proposed method. This is a more conservative approach, which is not as general as the first method. However, this method is specially useful when the developer think that a possible cause of flakiness may be the interaction between the simulator and ADS.}

\rwcomment{R1C5}{When discussing the answers to the RQs, namely from Page 12 and on, I would
recommend breaking these apart into separate subsections to better distinguish
them. Further, I would suggest some quick sentence or few words summary of the
corresponding RQ as a reminder on what is the purpose of the RQ and to put the
answer into context. By the time I had reached reading RQ1-3, I had forgotten
what the RQ actually is, so a reminder like that would really help with
comprehension.}
\response{We have improved the presentation by dividing Section~\ref{sec:eval} into multiple subsections and using lists with proper indentation to present items. Also, we have added summary sentences as reminders when discussing the results for each research question.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage

\noindent\textbf{Reviewer \#2}
%\rwcomment{R2C1}{It presents the aim well. I think the only level ot detail  I am missing is details around the fitness function (as the values were a bit hard to grasp in the content) - you really NEED to read the related work at some places (to understand the comparision aspect).} \response{}

\rwcomment{R2C2}{I much appreciate the hard and soft definition of flakiness - but I wonder if that would hold over time, as it is a context dependent definition for this study, but- this is not a flaw, but just a consideration. }
\response{We appreciate your feedback. 
The concept of hard flakiness is common in the literature and is used for systems with binary pass/fail test outcomes. In addition, our study introduces the notion of soft flakiness, a novel concept in the literature. We believe that the notion of soft flakiness is not tied to our context and is applicable to situations where a continuous fitness function or measure is used to evaluate test outputs, a common occurrence in the testing of cyber-physical systems.}


%The hard flakiness definition is used in many other studies as cited in the related works section. Hard flakiness definition has applications for cases in which a pass/fail behaviour is only considered. However, our work formally introduces the soft flakiness definition concept for the first time in the literature. This concept is useful for applications in which we measure the performance with a continuous fitness function. For example, where we want to evaluate the ego-vehicle in case of keeping in the center of lane. In that case, although two ego-vehicles may not go out of the road, however, the one with a smaller fitness function (closer to the lane in the mean) is more desired. In such applications, soft flakiness can help in more accurate evaluation of algorithms.}

\rwcomment{R2C3}{I found as far as I could tell that the the approach is sound - even if details are left out, I have no doubt to trust the authors on the simulation scenarios (now here - a replication package would be wonderful!) But I am assuming that some aspects  was part of a contest etc, there is fair game. 
The paper is sufficient transparent to reveal "enough" information. }
\response{Thank you for the comment and your trust. We have provided the links to our complete replication package and supplementary material in Section \ref{sec:data} and on \referenceaddressed{R2C3L1}.}

\rwcomment{R2C4}{It is a well motivated study, that I find will be a significant contribution to the field. I have not given full marks for presentation - even if the mix of tables, models and text - and the flow is great! It was simply a bit heavy as someone outside the ADS field, have to strain a bit with related work to be able to fully enjoy it. I think stylistically - simple "borders" around definitions and key aspects might help. I would not mind one more page added, where you bring in the tools in a short summary (+ and -) or a table for that so references had not to be checked.}
\response{Thank you for your comments. We have now improved the overall readability of our paper: (1) We revised and ensured the readability of all figures, tables, and algorithms. (2) We divided Section~\ref{sec:eval} into multiple subsections and used lists with proper indentation to present items. (3) We added Table~\ref{tab:expinfo} to clearly describe the characteristics of the ADS test setups used in our experiments. (4) We included summary sentences in the evaluation section to enhance readability. (5) We addressed all presentation issues raised by the three reviewers. (6) We have added a table (Table~\ref{tab:finalres}) to our discussion (Section~\ref{sec:conclusion}) to summarize the results that are used as a basis to derive our two main lessons.}

\rwcomment{R2C5}{Also I would prefer a bit more detail (as said) on the fitness funcitons used  - it is a bit summaric "calculate fitness" is not really replicatable.  - also what fuzzing was used  (or did I misunderstand? - you mean it is common to use it?).}
\response{We have now added discussions detailing the implementation of the random testing algorithms used for our experiments on \referenceaddressed{R2C10-1}. Further, we have  augmented and improved the description of the fitness functions used in our experiments on \referenceaddressed{R2C10-2}.}

\rwcomment{R2C6}{Soundness, significance and novelty is met, it is verified sufficiently, but transparency is the area I am thinking could be better. Therefore the length is slightly to short, as adding these details would benefit the paper being more self-contained. }
\response{We have provided a detailed and complete  replication package online~\cite{github}. In addition, as described in \comm{C12}, we have expanded the discussions related to the definitions of fitness functions and random testing. Finally, as discussed in \comm{C11},  we have considerably improved the presentation of our paper to provide a clearer and more comprehensive explanation of the various aspects of our experiments.}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage

\noindent\textbf{Reviewer \#3}

\rwcomment{R3C1}{The authors have been using the CARLA and BeamNG as simulators. Given the amount of possible flakiness reported and the examples of flaky behavior raise doubts whether the tools or models really are relevant for the ADS industry. The tools are claimed to be widely used, but by whom? The authors need to convince the reader a bit more.}
\response{CARLA and BeamNG are widely-used open-source simulators for ADS testing. They both have been used in several recent research on ADS testing, e.g.,~\cite{samota,zhong,haq2022manyobjective}. The software testing research community has established competitions based on BeamNG and has used this simulator to benchmark different testing approaches~\cite{beamng,sbftgithub}. CARLA has received endorsements from large companies such as Benz, Huawei, and Samsung~\cite{carlawebsite}, and is sponsored by Intel, NVIDIA, and Toyota~\cite{carlaservices}. According to a recent literature survey BeamNG and CARLA are the two top open-source simulators that can be flexibly  used for different levels of virtual and hybrid testing and have been widely referenced in the ADS testing literature~\cite{wherearewe}. 
Finally,  we note that potential flakiness of simulators for robotics and cyber-physical systems is a known problem. A recent industry survey lists simulation flakiness as a major challenge for robotic simulators~\cite{afsoon-robotics}.\\ %Considering the extensive use of CARLA and BeamNG in current research, dismissing our work for using these two simulators would suggest that a vast body of existing research is also irrelevant.\\ %While advanced commercial ADS simulators are available, their prohibitive costs often deter their widespread use in the academic literature.\\
That being said, we would like to emphasize that our study's findings are not meant to criticize BeamNG and CARLA. As we discuss in Section~\ref{sec:conclusion} under the \emph{Clarification of the Scope} item, many factors may contribute to the flakiness of simulators. Some of these factors, such as uncertainties in the physical models of simulators, are inherent to the physics-based design of both commercial and open-source simulators, and hence may be inevitable. \\
Instead, our results indicate that the methods employed in the software engineering literature for assessing simulation-based ADS testing approaches may  lack robustness and may be unreliable  due to the flakiness of ADS simulators. Specifically, the literature relies on the number of individual failing test scenarios and the values of fitness functions as metrics to evaluate testing approaches~\cite{haq2022manyobjective,samota,sbftgithub,raja2018}. Our experiments, which are grounded in existing ADS test setups from the literature ~\cite{haq2022manyobjective,samota,sbftgithub}, demonstrate that the values of these metrics  can exhibit significant nondeterminism.  As we discuss in Section~\ref{sec:conclusion} under the \emph{Implications of Our Results} item, we either need to consider restricted ADS test setups where the flakiness is negligible, e.g. the \textsc{Comp} setup in our study, or we need to develop an evaluation  method that is not sensitive to flakiness. We have updated our paper with a summary of this discussion on~\referenceaddressed{R3C1-intro}.}


%For example,  in scenarios where our evaluation is dependent on fitness function values and the count of individual failing test cases, we can easily surpass the performance of a given testing approach A by simply re-executing every candidate test in A multiple times. 


%For the BeamNG, as \cite{??} states, it is the most widely used Simulator in recent ADS development researches and competitions such as \cite{sbftgithub}. According to the results of a study based on a combination of surveys and interviews, CARLA is among the top tools used for testing ADS ~cite{https://dl.acm.org/doi/pdf/10.1145/3540250.3549111}. A recent systematic literature review identifies both CARALA and BeamNG among the the only  open source tools that support different levels of testing for autonomous cars and are the most cited open source tools in the literature https://arxiv.org/pdf/2206.05961.pdf


\rwcomment{R3C2}{The investigation uses four very basic requirements. Is that a good number? Are they representative for typical tests of ADS or are they oversimplified compared to requirements of a commercial ADS system? The use of fitness functions is very straight-forward, but is dependent on the requirement and thus gives very different ranges which might be hard to compare. For instance, the distribution of the fitness values can be very different.
}
\response{Thank you for the comment. We ground our experiments on  existing ADS test setups from the literature ~\cite{haq2022manyobjective,samota,sbftgithub}. Our \textsc{Pylot} and \textsc{Tran} setups are, respectively, replications of the ADS test setups from~\cite{haq2022manyobjective} and~\cite{samota}, and use the same four requirements described in the original setups. Our \textsc{Comp} setup is based on the the SBFT competition benchmark~\cite{sbftgithub} and considers one requirement as consistent with the SBFT benchmark. Hence, the choice of these four requirements, the description of the requirements,  the specification of input variables,  the definition of fitness functions, and even the baseline random testing  are taken from the  online replication packages of these three studies~\cite{haq2022manyobjective,samota,sbftgithub}. Regarding \textsc{PID} and \textsc{BeamNG}, the two setups introduced in our paper, we have ensured their consistency with \textsc{Pylot} and \textsc{Tran}.  \\
Considering extra requirements not present in the original studies, while a straightforward task, contradicts our core objective of replicating existing work to evaluate the presence of any flakiness in their results. Further, it is important to note that these four requirements, which encompass collision and lane keeping safety functions, are regarded as the essential safety requirements for ADS~\cite{wherearewe}.  \\
Regarding the sensitivity of our results to different ranges for fitness functions, we note that  we have normalized the ranges of the fitness functions to be able to compare them. Further,  our point in this papers is that flakiness can lead to variations to fitness values across different re-runs. Observing variations is  independent of fitness value ranges.  Given that we assess flakiness after normalizing the fitness functions, we believe that our analysis is not impacted by differences between fitness functions ranges.  We have provided detailed explanations and clarifications on how our fitness function definitions and implementations align with the existing setups documented in the literature on~\referenceaddressed{R2C10-2}. In addition, we have now discussed the above points in the threats to validity discussion in Section~\ref{sec:threats}.  Further details are provide in our replication package~\cite{github}.}

\rwcomment{R3C3}{Page 3, starting at line 33 the authors note that the flakiness in their investigation is on par with those observed in testing of software code. Why is this an important fact?}
\response{Flakiness is considered an important challenge for testing software code. Our study shows that test flakiness can arise in ADS test setups with a comparable frequency and significance. However, since this sentence is not used anywhere in our paper, and our results and arguments are in no way related to this sentence, we have now removed this sentence from our paper (see~\referenceaddressed{R3C3int}).}

\rwcomment{R3C44}{Page 8, line 14. How do the authors justify their definition of SF? Wouldn't some kind of variance function be a more obvious candidate? }
\response{Thank you for the comment. 
For soft flakiness, the key attribute a metric should possess is the ability to capture the degree of variations in fitness function values across multiple re-runs. Our current choice for the SF metric, i.e, the difference between max and min, maintains the metric's scale consistent with that of the fitness function, facilitating easier interpretation.
While we acknowledge variance as a potential alternative for the SF metric, it presents a challenge due to its squared scaling of the fitness function values. In other words, if the differences between the fitness values and the mean exceed one, the variance will be greater than the mean of these differences; and dually, if these differences are less than one, the variance will be smaller.   This scaling inconsistency complicates the interpretation of an SF metric measured by variance, as the metric values do not align with the scale of fitness values. We have added this discussion to the threats to validity discussion in Section~\ref{sec:threats} on~\referenceaddressed{R3C44ll}.} 

\rwcomment{R3C4}{Page 8, line 37. The authors suggest that by removing abnormal re-executions, some flaky tests might become non-flaky. How can this happen? If a test can generate abnormal re-executions, isn't that a flaky behavior and need to be attained?}
\response{Thank you for the comment. The purpose of this sentence was to  motivate RQ1-2. We realize that more clarification and context is needed for that sentence. We have updated the text as follows: A possible strategy can be to discard test re-executions exhibiting extreme abnormalities. For example, Figure~\ref{fig:figflakyhard}(c) shows a test re-execution with extreme abnormality, while the test re-execution in Figure~\ref{fig:figflakyhard}(b) looks normal. Eliminating abnormal cases may mitigate flakiness if the majority of flaky ADS tests consist of occasional major abnormalities among predominantly normal and consistent re-executions. However, if most re-executions are normal  but still exhibit noticeable variations, such as the example in Figure~\ref{fig:figflaky}, this approach will not be effective. We pose the RQ1-2 question to determine if most flaky tests are categorized by consistent normal re-executions with occasional extreme abnormalities, or if they exhibit variations but with few extreme abnormalities. The above update is applied to~\referenceaddressed{R3C4ll}. In addition, we have restructured the discussion after the RQ1 question so that each sub-RQ of RQ1 appears right after the paragraph motivating that sub-RQ. 
}

%These are for cases that something went wrong in the backend of the simulator such as cases that the ego-vehicle suddenly ended up being in the sky. Although these are actually flakiness by the definition, however, they can be easily mitigated by removing them from the simulations. In some cases, after removing such experiments, the scenario was not flaky at all.}

\rwcomment{R3C5}{Section 4 is describing the investigations in text. For clarity it would be beneficial to accompany the text with a table showing the experiment design in terms of variables and configurations.}
\response{We have now added Table~\ref{tab:expinfo} to clearly describe the characteristics
of the ADS test setups used in our experiments. Further, we have summarized some of the most important results of the paper in Table~\ref{tab:finalres}. 
Finally, we have revised Section~\ref{sec:eval}, and ensured the readability of all figures, tables, and algorithms.}

\rwcomment{R3C6}{Section 4 covers both the test setup and the results. Wouldn't it be better to make a new section at page 12, line 12 called Results?}
\response{Thank you for the comment. We  have now  divided Section~\ref{sec:eval} into multiple subsections to improve readability.}

\rwcomment{R3C7}{Page 10, starting line 19. It is written that Algorithm 3 determines the number of required re-runs. The only output from Algorithms 3 is fopt.}
\response{Thank you for the comment. We have now revised and clarified that sentence as follows: Algorithm~\ref{alg:smartfitnessn} uses predictions of ML classifiers to \emph{minimize} (and not determine) the number of required reruns. In other words, Algorithm~\ref{alg:smartfitnessn}, instead of re-running each test an equal number of times, reruns a test only until we can infer it is flaky. See~\referenceaddressed{R37alg3} }

\rwcomment{R3C8}{It is good that the costs of running the experiments are there provided n RQ1-1. This could also be done for all investigations and followed up in the discussion. We need to understand the proportions. Is retraining of a machine learning algorithm more resource consuming than running 1 000 simulations?}
\response{Thank you for the comment.  Simulations are the most time-consuming element of our experiments. A single simulation can take a minimum of one minute and may even take several minutes for some setups. In contrast, training machine learning techniques for our \textsc{STEC} and \textsc{MTEC} using a few thousands of data points takes less than a minute. Hence, the time spent training machine learning models in our experiments is quite negligible compared to the time required to run 1000 simulations, with ten repeats for each test setup, a process that can span from several days to a few months. A further clarification is that we do not re-train the \textsc{STEC} and \textsc{MTEC} models in Algorithm~3. These models are trained only once and used in Algorithm~3  only for inference.}

 

\rwcomment{R3C9}{In Table 1 there are some   combinations that end up in non-negligible soft flakiness and some does not. Yes, but what do we learn from this? Are the results expected? Shall we avoid certain combinations in the setup? }
\response{This table, which is now Table 2 in the paper,  shows that all test setups exhibit non-negligible soft flakiness for at least one of their fitness functions.  Regarding what we learn from this table, we have included three lessons in Section~\ref{sec:conclusion}: (1)~The lane-keeping test setup shows the lowest rate of flaky tests, (2)~Modular DNN-enabled ADS reduces flaky tests compared to  end-to-end DNN-enabled ADS, and (3)~The Carla simulator yields a lower flaky test  rate compared to the BeamNG simulator.  These three lessons build on the findings from Table~2 and Table~3. See~\referenceaddressed{R1C7L1}.
}

\rwcomment{R3C10}{Page 22, starting line 49 The authors comment on RQ1-1 that there is a difference between BeamNG and COMP. But BeamNG has generally a very high proportion of hard flaky tests compared to the other setups as well. A comment about this would be valuable.}
\response{To address this comment, we have now added a new lesson to Section~\ref{sec:conclusion} stating that based on our findings the BeamNG simulator shows a higher degree of flakiness compared to CARLA. See~\referenceaddressed{R3C10ll}}

\rwcomment{R3C11}{RQ1-2 Is a good complement to the automatically generated data. It also serves as some kind of grounding of the fitness functions, which is definitely needed. One small question, were the decisions about classification of the videos made by consensus among the viewers or was there a voting?}
\response{For RQ1-2, the classification of the variations listed in Table~\ref{tab:variations-carla} was determined by a consensus among the authors.}
%one of the co-authors watched PID setup videos and the other co-author watched Pylot setup videos. Each co-author wrote down important details and causes of flakiness on each scenario videos. After that, all co-authors had a discussion and considered their foundings and classified them into Table \ref{tab:variations-carla}.}

\rwcomment{R3C12}{The results of RQ1-3 are very much expected. Is this even necessary for the paper? One radical suggestion is to simply remove it. Alternatively, create a better justification and discussion about the results. }
\response{We believe RQ1-3 is an important research question that assesses the \emph{scale} of the impact of flaky tests on ADS testing. 
We have improved the question and its justification. The question is now stated as follows: \emph{Can the variations caused by flaky tests substantially impact the results of ADS testing algorithms?}
While the presence of flaky tests means that rerunning the same test is likely to impact the results of ADS testing algorithms, ideally, the magnitude and significance of this impact should be minimal.
RQ1-3 shows that this impact is statistically significant with a large effect size for at least two fitness functions of each test setup. We think these results are important and unexpected. See the updated text on~\referenceaddressed{R3C12ll}.}

%The results of RQ1-3 are directly related to the extent of flakiness of the simulator and test setup. So, for a highly deterministic simulator and test setup, re-running experiments should not make any or a huge difference. Therefore, we should investigate each simulator and test setup using RQ1-3 if don't know whether it's flaky or not beforehand. Based on this discussion, we believe the answer of RQ1-3 is not only unexpected, but also counter-intuitive since our paper is the first to investigate flakiness in ADS testing. This shows that many in the community were considering simulators as not a significant source of flakiness.}

\rwcomment{R3C13}{Table 9: What does A12 stand for?}
\response{$\hat{A}_{12}$ is the Vargha Delaney effect size. We have now clarified this point in the captions of 
Tables~\ref{tab:stattest} and \ref{tab:rq2-2-stattest-baseline}.}

\rwcomment{R3C14}{Validity threats is too short. For instance, the fitness functions mean different things to different requirements. Are the authors sure that the selected variable for measuring the fitness of each requirement is the correct one?}
\response{We have substantially expanded the discussion on threats to validity in Section~\ref{sec:threats}, using, among others, the responses to the comments received on our manuscript.}

\rwcomment{R3C15}{Page 21, starting line 15. The authors claim that their purpose is to investigate the potential causes of flakiness in ADS testing. But on page 22 starting line 25 authors write that it is not possible to assert which of the issues were the root causes of flakiness with the data from the paper. This is a contradiction.}
\response{Thank you for the comment. We have now updated the sentence in the \emph{threats to validity} discussion to be consistent with our statement of contributions as follows: \emph{\ldots to study the prevalence of flaky tests in ADS simulation-based testing, their impact on test results of ADS  and ways to mitigate this impact.} See~\referenceaddressed{R3C15ll}.
}





==> answerMinorRevision.tex <==
\noindent\textbf{Associate Editor}
\vspace*{.5cm}
\rwcomment{ARC1}{ References should be cited in the text by name and year in parentheses; moreover, the list of references must be alphabetized by the last names of the first author of each work; please check the guidelines for authors on the journal’s webpage.}
\response{We have corrected the formatting for the refereces in the paper. }

\rwcomment{ARC2}{Reviewer 1 suggests having the “Discussion” before the “Related Work”. I somewhat agree with this proposal but leave it up to you whether you want to follow this suggestion.}
\response{We have moved the discussion section before the related work section. }



\newpage

\noindent\textbf{Reviewer \#1} 

\rwcomment{R1C1}{The paper now states that it does not observe non-determinism during the ADS
inference phase, which I believe means that when the model is run on the same
input twice it always give the same output prediction. I would like the paper
to explicitly clarify how exactly it observed this behavior, e.g., was the
model run many times on the exact same input to see whether it can make
different predictions? Further, it seems then that if the non-determinism is
not coming from the ADS model inference, then it must be that the inputs the
model observes is non-deterministic, namely that the simulator provides the
differing inputs. Can the paper make a statement that it observed the model
receiving differing inputs from run to run, reinforcing that the
non-determinism is solely in the interactions with the simulator?}
\response{The deterministic characteristic of our selected ADS models is due to the fact that they are based on deterministic components. In other words, there is no stochastic component in our ADS models. For example, our classic PID-based ADS model is based on PID controllers which is deterministic. Similarly, our modular-based and end-to-end ADS-DNNs exclusively contain deterministic layers, such as convolutional and dense layers. Therefore, given a fixed input, our ADS models always generate the same output.}



%\rwcomment{R1C2}{The new three findings added to the Discussion section are branded as lessons, but they feel more like interesting observations instead. I feel like for them to be treated as lessons, the paper should make some explicit statements on what actions are recommended for developers based on those findings. For example, "Lesson 1" discusses how COMP leads to a lower flaky test rate due to a restricted environment, so is a lesson here that developers should apply more restrictions of sorts to mitigate flakiness? Or is there some other action to recommend for developers? It would be good to tie in these observations and recommended actions then to the later subsection about "Implications of our results for future research on simulation-based ADS testing" in the Discussion section, which would better reinforce these implications.}

%\response{}


\rwcomment{R1C3}{Citations in text should be in sorted order, e.g., "[5, 24, 7, 9]" should be "[5, 7, 9, 24]"}

\response{We have corrected the formatting for the refereces in the paper. }


\rwcomment{R1C4}{Concerning paper structure, I think Discussion section should be moved to before Related Work section.}

\response{We have moved the discussion section before the related work section. }

==> authors.tex <==
\author{Shervin}
\email{}
\affiliation{%
\institution{University of Ottawa}
  \streetaddress{800 King Edward Avenue}
  \city{Ottawa}
  \postcode{ON K1N 6N5}  
  \country{Canada}
}




\author{Shiva}
\email{snejati@uottawa.ca}
\affiliation{%
  \institution{University of Ottawa}
  \streetaddress{800 King Edward Avenue}
  \city{Ottawa}
  \postcode{ON K1N 6N5}  
  \country{Canada}
}


\author{Claudio}
\email{}
\affiliation{%
  \institution{University of Luxembourg}
  \streetaddress{29 Avenue John F. Kennedy}
  \city{Luxembourg}
  \postcode{1859}
  \country{Luxembourg}
}



==> letterMajorReview.tex <==
\hfill\today

\vspace{1cm}

\noindent Dear Editor,

\vspace{1cm}


\noindent Enclosed please find a revised version of manuscript  \textbf{EMSE-D-23-00310}, titled \emph{``Evaluating the Impact of Flaky Simulators on Testing Autonomous Driving Systems''}. The manuscript is authored by 
Mohammad Hossein Amini (University of Ottawa), 
\hbox{Shervin Naseri} (University of Ottawa), 
and
\hbox{Shiva Nejati} (University of Ottawa).
We submitted the first version of the manuscript on July 24, 2023.\\

On October 2, 2023, we received a decision regarding the manuscript, indicating that a major revision was required. We are grateful to the reviewers for their excellent suggestions for improvement. We believe we have addressed all of the reviewers' comments as we detail in our responses provided alongside this letter.\\



\noindent In our responses,  each comment is followed by an explanation which is either a clarification or a description of the  changes we made in the manuscript to address the comment.
The comments are highlighted in red, while our responses are highlighted in blue.\\ %We indicate \emph{how} and \emph{where}  each comment has been addressed in the manuscript. \\

%We identify each comment with a label in the format \fcolorbox{black}{yellow}{\bfseries\sffamily\scriptsize Cn}, where n is an incremental number used for reference  in the manuscript.\\

\noindent For clarity, we attach two identical versions of the manuscript---one with highlights and one in a finalized, ``clean'' form.  \\


%\vspace{1cm} 

\noindent Thank you for considering our manuscript.\\[2em]
 \noindent
Sincerely,\\[.5em]
Mohammad Hossein Amini, \hbox{Shervin Naseri},  \hbox{Shiva Nejati}
\clearpage

==> letterMinorReview.tex <==
\hfill\today

\vspace{1cm}

\noindent Dear Editor,

\vspace{1cm}


\noindent Enclosed please find a revised version of manuscript  \textbf{EMSE-D-23-00310}, titled \emph{``Evaluating the Impact of Flaky Simulators on Testing Autonomous Driving Systems''}. The manuscript is authored by 
Mohammad Hossein Amini (University of Ottawa), 
\hbox{Shervin Naseri} (University of Ottawa), 
and
\hbox{Shiva Nejati} (University of Ottawa).
We submitted the first version of the manuscript on July 24, 2023.\\

On Nov 22, 2023, we received an accept with final edits decision regarding the manuscript. We are grateful to the reviewers and our associate editor for their excellent suggestions for improvement. We have addressed all the requested final edits in the paper.\\



%\noindent In our responses,  each comment is followed by an explanation which is either a clarification or a description of the  changes we made in the manuscript to address the comment. The comments are highlighted in red, while our responses are highlighted in blue.\\ %We indicate \emph{how} and \emph{where}  each comment has been addressed in the manuscript. \\

%We identify each comment with a label in the format \fcolorbox{black}{yellow}{\bfseries\sffamily\scriptsize Cn}, where n is an incremental number used for reference  in the manuscript.\\

%\noindent For clarity, we attach two identical versions of the manuscript---one with highlights and one in a finalized, ``clean'' form.  \\


%\vspace{1cm} 

\noindent Thank you for considering our manuscript.\\[2em]
 \noindent
Sincerely,\\[.5em]
Mohammad Hossein Amini, \hbox{Shervin Naseri},  \hbox{Shiva Nejati}
\clearpage

==> tex/acknowledgments.tex <==
\section*{Acknowledgment}



==> tex/approach.tex <==
% !TEX root =  ../main.tex
\section{Approach}\label{sec:approach}


==> tex/forJournal.tex <==
% Extra useful text that did not fit in the confernece version. To be used in the journal version. 


\emph{CARLA simulator.} CARLA, developed by Intel Lab~\cite{carlapaper}, is a free, open-source autonomous driving simulator that enables high quality ADS simulations through  a variety of digital assets like urban layouts, buildings, and vehicles~\cite{carlafoundations}. 

\emph{BeamNG simulator.} BeamNG is a versatile and comprehensive simulator with a custom physics engine. It is used as a scenario-based testing environment for autonomous driving applications~\cite{beamng}.


\emph{PID Controller-Based ADS.} We use CARLA's Traffic Manager as a classic PID-based ADS. We refer to this ADS as PID in the remainder of this section. PID performs the motion planning with a PID controller. The controller estimates the throttle, brake, and steering input needed to reach the destination. The PID controller has parameters for the proportional, integrator, and the derivative parts which can be modified~\cite{carlatm}. 


\emph{Pylot.} Pylot is a  modular, DNN-enabled ADS that uses  a publish/subscribe inter-module data transmission. %The modules form a directed acyclic graph, each serving as a node. Inputs are from a telephoto camera, a wide-angle camera, LiDAR, and GPS provided by a simulator (CARLA in our work).  Pylot's perception layer includes a module for traffic light detection, which receives data from the telephoto camera, as well as modules for traffic sign detection, lane detection, object detection, and tracking, which receive RGB images from  the wide-angle camera. GPS data is utilized for mapping and combined with LiDAR data for localization. The motion prediction module receives these inputs and the perception layer's output to provide the planning layer. The planning layer uses this information to determine desired waypoints for the ego-vehicle through route planning, behavior planning, and trajectory planning. 


\emph{Transfuser.} Transfuser is an end-to-end multi-modal ADS, taking an RGB image from a wide-angle camera and a representation of the LiDAR data to produce the desired commands for the controller. %Bear in mind, that the GPS coordinates of the intermediate waypoints and the goal location (relative to the ego-vehicle) are fed as input to the GRU in the model.\textcolor{blue}{still not sure what waypoints are? Maybe they should be introduced in Section 3. Also what is GRU?}


\emph{Traffic lights.} Each traffic light has a duration, which may randomly change in different re-executions of the same test input, for being green, red or yellow. To avoid randomness in traffic lights' behaviour, we  set the initial traffic lights' status and control the duration of  red, green or yellow using a constant random seed.  By using the same random seed for each re-execution, we eliminate this known randomness and ensure consistency in multiple re-executions of the same test input.

==> tex/probdesc.tex <==
% !TEX root =  ../main.tex
%\section{Simulation-based Testing of ADS}
%\label{sec:problem}
%There are a variety of free and commercial simulators for ADS. These simulators vary in the way they capture the physics-based concepts, and may differ in several technical aspects. However, we can employ them for testing ADS in a common way as demonstrated in the literature~\cite{??}. In particular, there are several automated testing frameworks for ADS that use ADS simulators such as PreScan~\cite{??}, CARLA~\cite{??}, BeamNG~\cite{??},  ProSiVIC~\cite{??} and SVL~\cite{??}. Before we describe the test automation in this context, we describe the terms scene and scenario have been commonly used in the literature on ADS testing and are defined as follows: \emph{Scene} is a snapshot (frame) in the simulation~\cite{??}. A scene is characterized by the detailed properties by mobile objects, surrounding objects, roads and the ambient conditions. \emph{Scenario} is ``the temporal development between several scenes in a sequence of scenes''~\cite{??}.  Figure~\ref{fig:concept} shows the conceptual overview of the elements involved in ADS testing using simulators. Specifically, the test input is  a \emph{configured} initial scene together with the maximum duration of the simulation and the timestep duration, i.e., the time duration between each two consecutive scenes in a scenario. By configured initial scene, we mean that some additional information is provided as to how objects behave during the simulation. In particular, the test input typically describes the initial and end points for the ego vehicle.  The test output is a scenario that the simulator generates based on the initial scene. Provided with the scenario generated by the simulator, we are able to gather detailed logs about the progression of mobile objects during the simulation and define fitness functions that assess various described requirements of the system. 



%\begin{figure}[tb]
%    \centering
%    \includegraphics[width=0.4\textwidth]{concept.png}
%    \caption{Our concept model containing our inputs.}
%    \label{fig:concept}
%\end{figure}

%The configured initial scene includes the following elements: (1)~Mobile objects including an ego vehicle, non-ego vehicles, and pedestrians. (2)~Surrounding objects which include any non-mobile objects such as buildings, parked cars, etc. (3)~Roads that represent the road maps, shapes and conditions. (4)~The ambient conditions which include the weather condition, the time of the day, and the ambient light. Each of these concepts may have a number of attributes, some examples of which are shown in Figure~\ref{fig:concept}. 



%We examine two different autonomous driving systems in our paper, Pylot and Transfuser. Pylot is a modular system that passes data from each module to the next in a pub/sub manor. As such, each module in the pipeline can be interpreted as a node in a directed acyclic graph. It takes input from a telephoto camera, wide-angle camera, LiDAR and GPS, provided by Carla. The data from the telephoto camera is used for traffic light detection, while the RGB image from the wide-angle camera is passed to several modules, including the traffic sign detection, lane detection, object detection and tracking. The combination of all the above comprise our perception layer. GPS is then used for mapping, which is sent to the localization module along with LiDAR data. The motion prediction module receives this data and the output from the modules in the perception layer and sends its results to the planning layer, where a combination of inputs from these three modules are used for route planning, behaviour planning, and finally, trajectory planning which decides the desired waypoints for the ego-vehicle.
%Transfuser, on the other hand, is an end-to-end multi-modal model, taking an RGB image from a wide-angle camera and a BEV (Bird's Eye View) representation of the LiDAR data to produce the required waypoints for the controller. Bear in mind, that the GPS coordinates of the intermediate waypoints and the goal location (relative to the ego-vehicle) are fed as input to the GRU in the model.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{SUT1.pdf}
%     \caption{Overview of a simulation-based test setup for ADS.}
%     \label{fig:sut}
% \end{figure}





%put these in the figure. 
%(1)~Location, velocity, acceleration, and orientation for the ego car and every mobile object such as other vehicles, bikes and pedestrians. (2)~The surrounding objects and their properties. (3)~The road conditions and shape. (4)~The weather condition, the time of the day, and ambient light. The first scene of the simulation is referred to as the \emph{initial scene}. 

%Some of the properties in the initial scene remain constant during all the subsequent scenes in a simulation, and some properties change. We refer to the former as \emph{variable properties} and the latter as \emph{fixed properties}.  In ADS testing, the variable properties of a scene includes the location, velocity, acceleration, and orientation for the ego car and every mobile object, while other properties are typically fixed. Specifically, to test ADS,  we do not typically change the road condition, the weather or the ambient light situation within a single simulation scenario. 

%The set of properties (both fixed and variables) can be further decomposed based on the source that controls them. There are three sources that control scene properties: (i)~properties controlled by test inputs, (ii)~properties controlled by the ego vehicle (SUT), and (iii)~the properties controlled by simulator. Test inputs control a subset of the properties of the initial scene, but usually have no direct impact on the properties of the subsequent scenes within a simulation. The ego car controls the properties of the ego vehicle in all the scenes of a simulation scenario (except for the initial scene). Note that, the ego car operates in a closed-loop way, and at each scene, it acts upon the inputs it receives at the previous scene. The simulator often controls the properties of other moving objects. Depending on the simulator setup or its configuration, the properties of other moving objects may or may not change from one simulation to another. 


%There are a variety of free and commercial simulators for ADS. These simulators vary in the way they capture the physics-based concepts, and may differ in several technical aspects. However, we can employ them for testing ADS in a common way as demonstrated in the literature~\cite{??}. In particular, there are several automated testing frameworks for ADS that use ADS simulators such as PreScan~\cite{??}, CARLA~\cite{??}, BeamNG~\cite{??},  ProSiVIC~\cite{??} and SVL~\cite{??}. 

















%To define the test inputs to our system, we first need to examine the inputs for each model tested. These are Pylot and Transfuser, and although their inputs may differ in some aspects, there are commonalities that we will discuss (as presented in \ref{fig:concept}).

%Our inputs to \textit{Pylot} are determined by a vector of 13 values, that follow the rules of \cite{Haq:22}, with the exception of \textit{Presence of Trees} and \textit{Presence of Buildings} as they require custom builds of the simulator (i.e. Carla 0.9.10.1) and \textit{Road length}, which seems to be fixed. These inputs are as follows:

%\begin{enumerate}
%   \item {\textbf{Road Type} $\in \{Straight,\allowbreak Left turn, \allowbreak Right Turn, \allowbreak Cross Road\}$}   
%    \item {\textbf{Road ID} $\in \{0, \ldots, 3\}$}   
%    \item {\textbf{Vehicle in front} $\in \{False, True\}$}
    
%    \item {\textbf{Vehicle in adjacent lane} $\in \{False, True\}$}
    
%    \item {\textbf{Vehicle in opposite} $\in \{False, True\}$}
    
%    \item {\textbf{Vehicle in front two-wheeled} $\in \{False, True\}$}
    
%    \item {\textbf{Vehicle in adjacent two-wheeled} $\in \{False, True\}$}
    
%    \item {\textbf{Vehicle in opposite two-wheeled} $\in \{False, True\}$}
    
%    \item {\textbf{Time of Day} $\in \{Noon, Sunset, Night\}$}
    
%    \item {\textbf{Weather} $\in \{Clear, \allowbreak Cloudy, \allowbreak Wet, \allowbreak Wet Cloudy, \allowbreak Soft Rain, \allowbreak Mild Rain, \allowbreak Hard Rain\}$}
    
%    \item {\textbf{Pedestrian Density} $\in \{False, True\}$}
    
%    \item {\textbf{Vehicle Target Speed} $\in \{20, 30 , 40\} \it{km/h}$}
    
%    \item {\textbf{Driving Task} $\in \{\text{Follow road (straight)}, \allowbreak\text{ Take }1^{st}\text{ exit (right)}, \allowbreak\text{ Take }2^{nd}\text{ exit (left)}\}$}
    
%\end{enumerate}

%The initial coordinates of the ego-vehicle, chosen from pre-existing locations defined for each map, are decided by \textbf{Road Type} and \textbf{Road ID}. Based on the type of road, the authors have manually selected spots that adhere to that layout. For instance, in the case of a straight road, there are 4 possible initial locations, which we can cycle through via Road ID. It is important to note that of the 4 mentioned possibilities, two are in the map \textbf{Town 1} and the other two in \textbf{Town 3}.


%\textbf{Vehicle in front}, \textbf{Vehicle in adjacent} and \textbf{Vehicle in opposite} determine the existence of other vehicles in predefined locations (like above) wherever applicable. These parameters might not take effect if the layout does not allow for such a setting (e.g. a road with a single one-way lane). The \textbf{two-wheeled} options for these vehicles spawns a bicycle variant instead of a car.

%\textbf{Time of Day} affects the azimuth and lighting conditions, and \textbf{Weather} chooses one of the presets already defined in Carla, impacting properties such as precipitation, reflectiveness of the road, etc.

%\textbf{Pedestrian Density}, if true, spawns 18 pedestrians in predefined locations on the sidewalks. The authors of \cite{Haq:22} have disabled the movement of pedestrians.

%\textbf{Vehicle Target Speed} is the desired speed for our ego-vehicle that the controller tries to achieve.

%\textbf{Driving Task} is only applicable if the \textbf{Road Type} is set to \textbf{CrossRoad}. The goal location of the ego-vehicle is dependent on this parameter.

%On the other hand, the configurator for the \textit{Transfuser} takes files as input for \textbf{scenario} and \textbf{route}. The scenario file defines the possible scenarios and positions of the actors in the scene, whereas the route file is in charge of setting up a route through way-points; Weather and lighting parameters are also included in this file. Similar to our pipeline for Pylot, actors other than the ego-vehicle can be tagged as \textbf{front}, \textbf{left}, or \textbf{right}.

%In our unified concept model in \ref{fig:concept}, a generalized model of our inputs and outputs under both ADSs can be seen. Each scenario consists of some static and dynamic concepts; Pedestrians can fall under either category, stationary or moving based on our configurator setup. Some of the attributes have been explained above, and some have been added to better reflect the properties of each entity.














